Towards Transparent Robotic Planning via Contrastive Explanations

Providing explanations of chosen robotic actions can help to increase the transparency of robotic planning and improve users' trust. Social sciences suggest that the best explanations are contrastive, explaining not just why one action is taken, but why one action is taken instead of another. We formalize the notion of contrastive explanations for robotic planning policies based on Markov decision processes, drawing on insights from the social sciences. We present methods for the automated generation of contrastive explanations with three key factors: selectiveness, constrictiveness, and responsibility. The results of a user study with 100 participants on the Amazon Mechanical Turk platform show that our generated contrastive explanations can help to increase users' understanding and trust of robotic planning policies while reducing users' cognitive burden.

==> _Introduction.tex <==
\begin{comment}
Outline:

- Why need explanations? What are the state of the art in explainable AI? What are their limitations? (i.e., mostly focusing on simpler model, not drawing insights from social science).

- Why contrastive explanations? Insights from social science, what are the key factors? 

- Our work: based on MDPs (why?), how do we define critical states, selectiveness, responsibility, constrictiveness? 

- A brief paragraph describe our AMT study.
\end{comment}
In recent years, there has been a significant rise in the incorporation of AI decision-making systems in daily life. However, due to their complex nature, they mostly function as “black-boxes,” with lay-users having little understanding of the reasons how a decision is made or why an action occurs. This often leads to misunderstanding and mistrust of the system, which can further lead to problems caused by system misuse \cite{10.1007/978-3-319-99740-7_21}. Thus, there is an increasing need for these systems to explain their intermediate steps toward reaching a goal.

The creation of explanations for autonomous decision-making systems is not a new idea with the entire field of explainable-AI expanding rapidly \cite{BARREDOARRIETA202082, Gunningeaay7120, adadi_berrada_2018}. 
There has been a significant amount of work done in the field to increase the transparency of models, with new models employing techniques such as post-hoc model simplification and parameter relevance to provide explanation. Additionally, there has been a push to use models that are innately more interpretable, but these models often suffer in performance.


However, few models consider social science theories of explanation during generation. For example, Miller suggests humans prefer contrastive explanations, or explanations that revolve around counterfactuals \cite{miller2017explanation}. Specifically, humans tend to ask not why an event P happens, but why an event P happens instead of some event Q. Understanding this contrast of events is more important to the human user than statements of probabilities or lists of total causes. An explanation only needs to be sufficient for the context being asked for by a human user. When a contrastive explanation is generated it can employ several factors to improve the flow of information. In this paper, we define ``contrastive explanations'' to include responsibility (rating how important an action is in causing an event) \cite{Halpern10.1093/lpr/mgu020}, constrictiveness (numbering how many future possible actions than an action causes) \cite{GIROTTO1991111}, and selectiveness (choosing the most relevant events) \cite{miller2017explanation}. Different combinations of factors allow an explanation to control information specificity and support provided for events and actions.

\todo{MDPs have been widely used as a modeling formalism to represent abstract robotic mission plans~\cite{Thrun05}}
We use these explanatory factors to generate explanations for autonomous route planning applications. To do this, we employ MDPs, or Markov Decision Processes, which allow us to capture a complex system, for example a network of alleyways, and reduce it down into a more accessible form. Furthermore, using an MDP, we can model the non-deterministic nature of these systems and verify the effects of our project on that system are sound. Concerning an MDP, we define selectiveness as the reduction of the explanation to only the actions taken at the critical states. We define responsibility as the sum of an action's influence factors or the deviation in reachability probability with or without that action present. We define constricitiveness as how a chosen action affects the flexibility of the future route. Finally, we test the effectiveness of our explanations using an Amazon Mechanical Turk Study as explanations exist in a social realm and are not effective if they are not understandable and trusted by users.

\startpara{Contributions} We summarize the major contributions of this paper as follows:
\begin{enumerate}
    \item A formalization of and an algorithm for critical states in MDPs.
    \item A formalization of and an algorithm for selectiveness, responsibility, and constrictiveness for MDPs, and a way to generate contrastive explanations using them.
    \item A user study of contrastive explanation effectiveness and preference using the newly defined concepts of selectiveness, constrictiveness, and constrictiveness.
\end{enumerate}

\startpara{Related Work} When applied to AI-based systems, the finding of counterfactuals is often treated as a search or optimization problem \cite{Mittelstadt:2019:EEA:3287560.3287574}. However, a counterfactual must be relevant to the system context or it will not produce an explanation that is understandable for the user. Additionally, counterfactuals can be isolated through the use of modeling by providing concise descriptions of system behavior\cite{kim_muise_shah_agarwal_shah_2019, miller2018contrastive, han_katoen_berteun_2009,1f738812b52b4a4c98b49d6369c23124,Hayes10.1145/2909824.3020233}. Furthermore, explanation creation and policy transparency can be based in finding critical states, or the most important states, when reduction of the explanation is necessary \cite{huang2018establishing}.

The explanations provided by an AI-based decision-making system must deal with the significant trade-off between what the system is trying to accomplish and what the users need to understand the decisions made fully \cite{feng2016synthesis}. Balancing these trade-off increases system interpretability and user accessibility \cite{Lieaay6276}. So, when creating an explanation, all possible explanatory factors and support must be chosen carefully to maximize explaninee understanding and minimize explainee burden.

Explicitly, the generation of contrastive explanations through structured language templates has been done in work such as \cite{feng2018counterexamples}. However, none of the previous works have produced contrastive explanations from structured language templates using selectiveness through the identification of critical states, responsibility, and constrictiveness, even though social science points to these factors as valid ways to increase explanation effectiveness. 

==> _Preliminaries.tex <==
\subsection{Markov Decision Processes}
Formally, a \textit{markov decision process} (MDP) is a tuple $\M = (S, s_0, A, \delta, r)$ where: (i) $S$ is a finite set of states, $s_0\in S$ is an \textit{initial state}; (ii) $A$ is a set of actions; (iii) $\delta: S\times A\times S \to [0,1]$ is a transition probability function mapping each state-action pair to a probability distribution over $S$; (iv) $r =(r_{state}, r_{action})$ is a \textit{reward structure} comprising a state reward function $r_{state}: S \to \R_{\ge 0}$ and an action reward function $r_{action}: S \times \delta \to \R_{\ge 0}$. 

From a given MDP, we can find some \textit{infinite path} $IPath_\M$, which is defined as a sequence of states and action/distribution pairs $\sigma = s_0 \xrightarrow[]{a_0} s_1\xrightarrow[]{a_1}...$, where $\delta_\M(s_i, a_i, s_{i+1})>0 $ for all $i \in \N$. A \textit{finite path} $\rho = s_0 \xrightarrow[]{a_0} s_1 \xrightarrow[]{a_1} ...\xrightarrow[]{a_{n-1}} s_n$ is a prefix of an infinite path ending in a state, denoted by $FPath_\M$. Each path represents a execution of the system which the MDP is modeling. A \textit{policy} is a choice of what action to choose at each state. Formally, a policy is a function $\pi$ mapping every finite path $FPath_\M = s_0 \xrightarrow[]{a_0} s_1 \xrightarrow[]{a_1} ...\xrightarrow[]{a_{n-1}} s_n$ to an element $\pi(\rho) \in \delta_\M$.

\begin{example}
Based on the grid map in Figure \ref{fig:grid}, we can abstract away an MDP model shown in Figure \ref{fig:mdp}. Specifically, the MDP is defined with states visualized, actions of moving north, south, east, west and stop, and transitions are labeled by the arrows. We also designed a reward structure, where $r_{action}$ measure the total amount of distance needed to reach the destination, and $r_{state}$ keeps track of the distance traveled in risky (yellow) states. An example policy for this MDP is to always choose the action that leads to grey states, i.e. to always choose the public highway in the motivating scenario. There could be many more different policies, and one of the main motivation for this paper is to better explain the choice of one policy over others.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.35]{Figures/mdp_new.png}
    \caption{MDP Abstracted from the Grid Map}
    \label{fig:mdp}
\end{figure}
\end{example}

\subsection{MDP properties}
There are a variety of properties of MDPs, each with methods to perform probabilistic model checking. \cite{forejt2011automated} In this paper, we let $\rho$ to be one particular property and define $\rho_s$ to be the value of that property at state $s$. Due to the non-deterministic characteristic of MDPs, we usually have a maximum property value $\rho_s^{max}$ and a minimum property value $\rho_s^{min}$ at each state. Two of the most commonly used properties are probabilistic reachability and reward-based properties. 

% Given an MDP $\M$ and a policy $\pi$ for it, we can define a probability measure $Pr^\pi_\M$ over the set of infinite paths $IPath_\M$, which allows us to determine the probability with which certain events occur under policy $\pi$.

\textit{Probabilistic reachability} is a simple yet fundamental property. First, given an MDP $\M$ and a policy $\pi$ for it, we can define a probability measure $Pr^\pi_\M$ over the set of infinite paths $IPath_\M$, which allows us to determine the probability with which certain events occur under policy $\pi$. Then probabilistic reachability refers to the minimum or maximum probability, when starting from a given state $s$, of reaching a set of target states $T\subseteq S$. \cite{forejt2011automated} Formally, let $reach_s(T)$ be the set of all paths that start from state $s$ and contain a state from $T$, then the maximum and minimum reachability probability are defined as:
$$Pr_{\M,s}^{min}(reach_s(T)) \eqdef \inf_{\sigma \in Adv_M}Pr_{\M,s}^\sigma (reach_s(T))$$
$$Pr_{\M,s}^{max}(reach_s(T)) \eqdef \sup_{\sigma \in Adv_M}Pr_{\M,s}^\sigma (reach_s(T))$$

There are many \textit{reward-based properties} for MDPs, but the one we used in this paper is the \textit{expected cumulative reward to reach a target}. Given an MDP $\M$, state $s\in S$ and a set of target states $T\subseteq S$, the expected cumulative reward to reach $T$ from $s$ will be $E_s^{min}(F_r^T)$ or $E_s^{max}(F_r^T)$ where $F_r^T: IPaths \to \R_{\ge 0}$ is the random variable such that, for any path $\pi \in IPaths_\M$:
% $$\eqdef \begin{cases}}$$
\[
  F_r^T(\pi)  = 
  \begin{cases}
    \infty, \text{ if } s_i\not\in T \text{ for all } i \in \N\\
    \sum_{i=0}^{k_\pi^T - 1} (r_{state}(s_i)+r_{action}(s_i, a_i)), \text{ else}\\
  \end{cases}
\]
where $k_\pi^T = min\{k|s_k\in T\}$.

\begin{example}
For the constructed MDP model, if we are interested in how likely it is for state $s$ to reach the destination, we can check the maximum reachability probability, then we will have $\rho_s^{max} = Pr_s^{max}$. Or if we want to know the least average distanced traveled in risky alleys at state $s$, we can instead let $\rho_s^{min} = E_s^{min}(F_{r_{state}}^T)$, remember we defined $r_{state}$ to keep track of the distance traveled in risky states.

\end{example}
% \startpara{Definition 3 (Probabiliy measure)} Given an MDP $\M$ and a policy $\pi$ for it, we can define a probability measure $Pr^\pi_\M$ over the set of infinite paths $IPath_\M$, which allows us to determine the probability with which certain events occur under policy $\pi$. We can also use expected values $E_\M^\pi(\cdot)$, for example of a cost function over paths.

% \startpara{Definition 4 (Probabilistic Reachability)} Probabilistic reachability is a property of the MDPs, referring to the minimum or maximum probability, when starting from a given state $s$, of reaching a set of target states $T \subseteq S$. \cite{forejt2011automated} Formally, let $reach_s(T)$ be the set of all paths that start from state s and contain a state from T, i.e.:
% $$reach_s(T) = \{\pi \in IPath_{\M,s} | \pi(i) \in T \text{ for some } i \in \N \}$$
% The measurability of $reach_s(T)$ follows from the fact that $reach_s(T) = \cup_{\rho \in I}\{\pi \in IPath_{\M,s} | \pi \text{ has prefix } \rho \}$, where $I$ is the (countable) set of all finite paths from $s$ ending in $T$, and each element of this union is measurable. Then the maximum and minimum reachability probability can be computed as followed:
% $$Pr_{\M,s}^{min}(reach_s(T)) \eqdef \inf_{\sigma \in Adv_M}Pr_{\M,s}^\sigma (reach_s(T))$$
% $$Pr_{\M,s}^{max}(reach_s(T)) \eqdef \sup_{\sigma \in Adv_M}Pr_{\M,s}^\sigma (reach_s(T))$$

% \startpara{Definition 5 (Reward-based property)} Another property is the expected cumulative reward. Given an MDP $\M$, state $s\in S$ and a set of target states $T\subseteq S$, the expected cumulative reward to reach $T$ from $s$ will be $E_s^{min}(F_r^T)$ or $E_s^{max}(F_r^T)$ where $F_r^T: IPaths \to \R_{\ge 0}$ is the random variable such that, for any path $\pi \in \IPaths$:
% % $$\eqdef \begin{cases}}$$
% \[
%   F_r^T(\pi)  = 
%   \begin{cases}
%     \infty, \text{ if } s_i\not\in T \text{ for all } i \in \N\\
%     \sum_{i=0}^{k_\pi^T - 1} (r_{state}(s_i)+r_{action}(s_i, a_i)), \text{ else}\\
%   \end{cases}
% \]
% where $k_\pi^T = min\{k|s_k\in T\}$.

\subsection{PRISM Probabilistic Model Checking}
Model checking \cite{clarke2018model} is a verification method used to determine whether a system satisfies given requirements. We first construct and describe the system under inspection in some high-level modeling formalism such as MDP. Then, we specify the properties to be verified as logical formulas of temporal logic such as LTL. These properties can capture many different aspects of system behavior, from reliability to performance. PRISM \cite{KNP11} is a leading probabilistic model checking tool, which can construct system models exhibiting probabilistic behavior and check quantitative properties specified in temporal logic. We believe that PRISM is suitable for our modeling and evaluation of VM migration performance as the system administrators can not only probe into the quantitative characteristic of system behaviors but also understand the degree of credibility and reliability through verification results.

==> _motivating_example.tex <==
\begin{comment}
Among the many automatic decision-making systems that need human-understandable explanations, navigation is one example that has extensive use in daily life and needs deep understanding and trust from the users. 
\end{comment}

Consider the route planning for an autonomous vehicle navigating in a grid map as shown in Figure~\ref{fig:grid}.
There are three routes from the start (S) to the destination (D) highlighted in different colors. 
The red route takes the highways, which has the longest distance and the lowest risk of colliding with pedestrians and cyclists.
The blue route cuts through the urban roads, which has the shortest distance but the highest risk of incidents.
The green route has a mixture of highways and urban roads, which has the medium distance and the medium risk.

\todo{motivate selectiveness, constrictiveness, responsibility, language template}
One straightforward solution to the problem of explaining the motivating example is to list out the actions at each state, which we will call the ``naive explanation". Detailed it may be, this approach brings a large cognitive burden on the users, who oftentimes cannot digest this large amount of information. 


%\begin{figure}[htp]
%    \centering
%    \subcaptionbox{Navigation through alleys\label{fig:road}}{\includegraphics[scale=0.23]{"Figures/alley road map".png}}\hspace{0.1em}%
%    \subcaptionbox{Grid map\label{fig:grid}}{\includegraphics[width=1in]{"Figures/grid".jpeg}}
%    \caption{Motivating example: from real map to grid map}
%\end{figure}
% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.25]{"Figures/alley road map".png}
%     \caption{Motivating Example: Navigation in Alleyways}
%     \label{fig:road}
% \end{figure}

 \begin{figure}[ht]
     \centering
     \includegraphics[scale=0.15]{Figures/labeled_grid.jpeg}
     \caption{An example grid map for robotic planning. Green grids: start (S) and destination (D). Black grids: buildings. Red grids: dead-ends. Yellow grids: urban roads. White grids: highways. }
     \label{fig:grid}
 \end{figure}

 


%Consider the following situation: a robot wants to navigate in an old neighbourhood like the one shown in Figure \ref{fig:road}, but there are a range of possible routes. In particular, some routes are on the public highway, which is less risky but may be longer, while others may take a shortcut through the neighbourhood alleys, but can have a higher risk of colliding with pedestrians or cyclists. It is possible that in these scenarios, there will not be one specific ``best'' path, but rather choices with trade-offs. When the robot made a certain route planning decision, how can it explain the reasoning behind its actions to the users in an comprehensible manners?

%To attempt answering these questions, the situation was first captured in Figure \ref{fig:grid} as a grid map, where red blocks are dead-ends in the alley, yellow blocks are risky alley ways, and the outermost white blocks are on the public highway. As Figure \ref{fig:grid} shows, there are three main reachable routes highlighted in different colors. Among the three options, the red route always chooses the public highway, which is the safest but longest route. The blue route, by contrast, cuts through the neighborhood alleys and therefore has the highest risk of incidents whereas the shortest distance. The green route is the compromise in the middle, neither the shortest nor the safest. Suppose the robot chooses the red route instead of the other ones, how can the system explain its decision so that the users have the highest level of understanding, trust and preference?

% All the possible actions are mapped in arrows on the grid map. Based on the abstraction, we built an MDP model incorporating the information specified in Figure \ref{fig:mdp}.

% \begin{figure}[tp]
%     \centering
%     \subcaptionbox{grid map\label{fig:grid}}{\includegraphics[width=1.55in]{"Figures/grid".jpeg}}\hspace{0.4em}%
%     \subcaptionbox{mdp\label{fig:mdp}}{\includegraphics[width=1.55in]{"Figures/selective".jpeg}}
%     \caption{Abstraction based on the motivating scenario}
% \end{figure}

% Specifically in this example, the MDP has the following components:
% \begin{itemize}
%     \item States $S = \{(i, j) | 1\le i, j \le 5 \And (i,j) \ne (4,2)\}$
%     \item Actions $A = \{ N, S, W, E, Stop\}$
%     \item Transition probability $T$, specified by the arrows on each state in the grid map
%     \item Reward $R$, we have designed two reward structures including total\_dist to destination, risky\_steps to destination.
% \end{itemize}

% In this example, there are three main reachable routes indicated on the grid map in Figure \ref{fig:grid} with different colors. Among the three options, the red route always chooses the public highway, which is the safest but longest route. The blue route, by contrast, cuts through the neighborhood alleys and therefore has the highest risk of incidents whereas the shortest distance. The green route is the compromise in the middle, neither the shortest nor the safest.Suppose the robot chooses the red route instead of the other ones, the users may be confused why it does not take the blue route, which seems much shorter.

% One straightforward solution is to explain its actions at each state, which we will call the ``naive explanation" in the following section. Detailed it may be, this approach brings a large cognitive burden on the users, who oftentimes cannot digest this large amount of information. Therefore, we devise the ``selective explanation" which only explains at a handful of ``critical states". 

% Once the system knows where it explains, it needs to figure out what to explain at these states. In this paper, we defined two properties that we think is important for comparing various actions: ``constrictiveness'' and ``responsibility''. Constrictiveness essentially indicates the number of future decision points is left in the route that one action directs to. Usually, more decision points lead to more flexibility for the robot to reroute, hence less constrictive actions are preferred by the system as time passes. Responsibility refers to the likelihood that one action can reach the final destination. The higher the responsibility, the more probability that this action can reach the target states. We will discuss their definitions and the algorithms to compute them in detail in the next section. 

